A posteriori error estimates for the Electric Field Integral Equation on polyhedra

We present a residual-based a posteriori error estimate for the Electric Field Integral Equation (EFIE) on a bounded polyhedron. The EFIE is a variational equation formulated in a negative order Sobolev space on the surface of the polyhedron. We express the estimate in terms of square-integrable and thus computable quantities and derive global lower and upper bounds (up to oscillation terms).

==> defs.tex <==
\newcommand{\eT}{\mathcal E(T)}

\newcommand{\step}[1]{\noindent\raisebox{1.5pt}[10pt][0pt]{\tiny\framebox{$#1$}}\xspace}

%\newcommand{\parasym}{{\footnotesize ||}}
%\newcommand{\mesh}{{\mathcal T}}
\newcommand{\mesh}{{\mathcal T}}

%%% spaces %%%
\newcommand{\real}{{\mathbb{R}}}
\newcommand{\complex}{{\mathbb{C}}}
\renewcommand{\H}[1]{H^{#1}(\Gamma)}
\newcommand{\Hb}[1]{\bm H^{#1}(\Gamma)}
\newcommand{\Hpara}[1]{\bm H^{#1\frac12}_{\parallel}(\Gamma)}
\newcommand{\Hparas}[1]{\bm H^{#1}_{\parallel}(\Gamma)}
\newcommand{\Hortho}[1]{\bm H^{#1\frac12}_{\bot}(\Gamma)}
\newcommand{\Horthos}[1]{\bm H^{#1}_{\bot}(\Gamma)}
%\newcommand{\Hdiv}{\bm X^{-\frac12}_{{\rm div}}(\Gamma)}
\newcommand{\Hdiv}{\bm H^{-\frac12}_{{\rm div}}(\Gamma)}
\newcommand{\Hdivp}[1]{\bm H^{#1}_{{\rm div}}(\Gamma)}
\newcommand{\Hcurl}{\bm H^{-\frac12}_{{\rm curl}}(\Gamma)}
\newcommand{\HcurlO}{\bm H({\curl},\Omega)}
\newcommand{\hcurlo}{\bm H({\rm curl},\Omega)}
\newcommand{\Hloc}{\bm H^1_{{\rm loc}}(\Omega)}
\newcommand{\Hone}{\bm H^1(\Omega)}
\newcommand{\Lt}{\bm L_t^2(\Gamma)}
\newcommand{\lt}{L^2(\Gamma)}
\newcommand{\RT}{\bm {RT}_0}
\newcommand{\Hcal}{\mathcal H(\Gamma)}
\newcommand{\Hminus}[1]{\bm H^{#1\frac12}_{-}(\Gamma)}

%%% operators %%%
\renewcommand{\div}{{\rm div}_\Gamma}
\newcommand{\grad}{{\bf grad}_\Gamma}
\newcommand{\gradx}{{\bf grad}_{\Gamma,\x}}
\newcommand{\curl}{\boldsymbol{\mathrm{curl}} \; }
\newcommand{\curlv}{{\bf curl}_\Gamma}
\newcommand{\curls}{{\rm curl}_\Gamma}
\newcommand{\curlsx}{{\rm curl}_{\Gamma,\x}}
\newcommand{\lap}{{\Delta}_\Gamma}
\newcommand{\Ak}{\bm A_k}
\newcommand{\Vk}{V_k}
\newcommand{\Gk}{G_k}
\newcommand{\Ipsi}{{\mathbf I}_{\mesh}}
\newcommand{\Ialpha}{ {\rm I}_{\mesh}}
\newcommand{\SLPs}{\Psi^V_k}
\newcommand{\SLPv}{\bm \Psi^A_k}

%%% norms %%%
\newcommand{\nHdiv}[1]{\|#1\|_{\bm H^{-\frac12}_{\rm div}(\Gamma)}}
%\newcommand{\nHdivs}[3]{\|#2\|_{\bm H^{#1}_{\rm div}(#3)}}
\newcommand{\nHcurl}[1]{\|#1\|_{\bm H^{-\frac12}_{\rm curl}(\Gamma)}}
\newcommand{\nHortho}[2]{\|#2\|_{\bm H^{#1\frac12}_{\bot}(\Gamma)}}
\newcommand{\nHorthos}[1]{\|#1\|_{\bm H^{s}_{\bot}(\Gamma)}}
\newcommand{\nHDelta}[2]{\|#2\|_{\bm H_-^{#1}(\Delta_T)}}
\newcommand{\nHpara}[2]{\|#2\|_{\bm H^{#1\frac12}_{\parallel}(\Gamma)}}
\newcommand{\nHparas}[1]{\|#1\|_{\bm H^{s}_{\parallel}(\Gamma)}}
\newcommand{\nH}[2]{\|#2\|_{H^{#1}(\Gamma)}}
\newcommand{\nHb}[2]{\|#2\|_{\bm H^{#1}(\Gamma)}}
\newcommand{\nHbT}[2]{\|#2\|_{\bm H^{#1}(T)}}
\newcommand{\nHminus}[2]{\|#2\|_{\bm H^{#1\frac12}_{-}}}
\newcommand{\nLt}[2]{\|#1\|_{\bm L^2({#2})}}
\newcommand{\nlt}[2]{\|#1\|_{L^2({#2})}}

%%% scalar products %%%
\newcommand{\para}[2]{\langle #1, #2\rangle_{\parallel,\Gamma}}
\newcommand{\Ltwo}[2]{\langle #1, #2\rangle_{0,\Gamma}}
\newcommand{\LtwoT}[2]{\langle #1, #2\rangle_{0,\ka}}
\newcommand{\half}[2]{\langle  #1, #2\rangle_{\frac12,\Gamma}}
\newcommand{\threetwo}[2]{\langle  #1, #2\rangle_{\frac32,\Gamma}}
\newcommand{\halfk}[2]{\langle  #1, #2\rangle_{\frac12,\ka}}
\newcommand{\ortho}[2]{\langle  #1, #2\rangle_{\bot,\Gamma}}
\newcommand{\po}[2]{~\hspace{-0.2cm}_\bot\!\langle #1, #2\rangle_{\parallel}}
%\newcommand{\aa}[2]{a(\bm  #1,\bm #2)}

%%% variables %%%
\renewcommand{\u}{\bm u}
\renewcommand{\v}{\bm v}
\newcommand{\w}{\bm w}
\newcommand{\uh}{\bm U}
\newcommand{\eh}{\bm E}
\newcommand{\vh}{\bm V}
\newcommand{\n}{\bm n}
\newcommand{\x}{\bm x}
\newcommand{\y}{\bm y}
\renewcommand{\r}{\bm r}
\newcommand{\f}{\bm f}
\newcommand{\Psiv}{\bm \Psi}
\newcommand{\Psivm}{\bm \Psi_\mesh}
\newcommand{\alpham}{\alpha_\mesh}
\newcommand{\dPsiv}{\delta\hspace{-1.2pt}\bm \Psi}
\newcommand{\dalpha}{\delta\hspace{-1.2pt}\alpha}
\newcommand{\Res}{\bm R}
\newcommand{\cres}{r}
\newcommand{\LRes}{\Res_{\ka}}
\newcommand{\Lcres}{\cres_\ka}
\newcommand{\LResG}{\Res_0}
\newcommand{\LcresG}{\cres_0}
\newcommand{\h}{{\tt h}}

%%% communication %%%
\newcommand{\todo}[1]{\noindent \color{red}{\bf TODO:} #1 \\\color{black}}
\newcommand{\rem}[1]{\noindent \color{red}{\bf REM:} #1 \\\color{black}}
\newcommand{\bs}[1]{\noindent \color{blue}{\bf BS:} #1 \\\color{black}}
\newcommand{\caut}[1]{\noindent \color{red}{\bf CAUTION:} #1 \\\color{black}}

%%% other %%%
\newcommand{\calI}{\mathcal I}
\newcommand{\edges}{\mathcal E_\mesh}
\newcommand{\nodes}[1]{\mathcal N(#1)}
\newcommand{\set}[2]{\left\{ #1\,\middle|\,#2\right\}}
%\newcommand{\gtrace}{\gamma_{\tau}}
%\newcommand{\ptrace}{\pi_{\tau}}
\newcommand{\gtrace}{\bm\gamma_{\perp}}
\newcommand{\ptrace}{\bm\gamma_{\hspace{2pt}\parallel}}%\shortparallel
\newcommand{\Rortho}{\bm R_{\perp}}
\newcommand{\Rpara}{\bm R_{\parallel}}%\shortparallel
\newcommand{\Rtrace}{\bm R_{\bm\gamma}}
\newcommand{\tperp}{\bm t_{\perp}}
\newcommand{\smspace}{\hspace{-0.1cm}}
\newcommand{\smtimes}{\smspace\times\smspace}
\newcommand{\ka}{T}

\newcommand{\de}{\,{\rm ds}}
\newcommand{\ds}{\,{\rm d}\sigma}
\newcommand{\dO}{\,{\rm d}\Omega}
\newcommand{\VP}{\mathbb V(\mesh)}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{figure}[theorem]{Figure}

